Simple and Scalable Strategies to Continually Pre-train Large Language Models

Large language models (LLMs) are routinely pre-trained on billions of tokens, only to start the process over again once new data becomes available. A much more efficient solution is to continually pre-train these models, saving significant compute compared to re-training. However, the distribution shift induced by new data typically results in degraded performance on previous data or poor adaptation to the new data. In this work, we show that a simple and scalable combination of learning rate (LR) re-warming, LR re-decaying, and replay of previous data is sufficient to match the performance of fully re-training from scratch on all available data, as measured by the final loss and the average score on several language model (LM) evaluation benchmarks. Specifically, we show this for a weak but realistic distribution shift between two commonly used LLM pre-training datasets (English$\rightarrow$English) and a stronger distribution shift (English$\rightarrow$German) at the $405$M parameter model scale with large dataset sizes (hundreds of billions of tokens). Selecting the weak but realistic shift for larger-scale experiments, we also find that our continual learning strategies match the re-training baseline for a 10B parameter LLM. Our results demonstrate that LLMs can be successfully updated via simple and scalable continual learning strategies, matching the re-training baseline using only a fraction of the compute. Finally, inspired by previous work, we propose alternatives to the cosine learning rate schedule that help circumvent forgetting induced by LR re-warming and that are not bound to a fixed token budget.

==> continual_learning_background.tex <==
\section{Continual Learning}
\subsection{Introduction}

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.6\textwidth]{intro_figs/data trends.pdf}
    \caption{Cumulative Common Crawl size on monthly basis}
    \label{fig:data-trends}
\end{figure}


As can be seen in the Fig. \ref{fig:data-trends}, the amount of data on common crawl, a free, open repository of web crawl data commonly used to train large language models, continues to grow every month. Currently the norm is to train from scratch on a new compilation of the data. However, this results in growing training computational costs as dataset sizes continue to grow. One approach to mitigate the increasing computation cost is to continually expand capabilities of foundation models by building upon existing knowledge and continuing to train instead of training from scratch. 

The goal of continual learning is to study and develop algorithms and strategies that allow learning from a sequence of non-stationary distributions and environments. It requires not only adapting quickly and learning new tasks, but also preservice knowledge from past tasks over the model’s lifetime. It is also referred to as incremental or lifelong learning. 

\subsection{Challenges of Continual Learning}
There two broad categories of challenges associated with continual learning mainly revolving around a trade-off between learning plasticity (ability to learn new data) and memory stability (ability to retain past knowledge) \cite{wang2023comprehensive}:

\begin{enumerate}
    \item Memory stability: This refers to the ability to retain past knowledge
    \begin{enumerate}
        \item  Catastrophic forgetting: This occurs when the model faces rapid decline in its performance on previous tasks when being trained on a new distribution or task. Algorithms such as Stochastic Gradient Descent (SGD), are designed to optimize learning the current training without any mechanism to preserve past knowledge outside of the current distribution. 
        \item Backward Transfer: This refers to the effect of learning a new task on all previous tasks 
    \end{enumerate}
    \item Learning plasticity: This refers to the ability to learn new knowledge
    \begin{enumerate}
        \item Intransigence: This represents the model inability to learn a new task. This occurs when training from scratch or training jointly results in better performance for the given task than continually training a model trained on previous tasks. 
        \item Forward transfer: This represents the influence of previous tasks on the new task.
    \end{enumerate}
\end{enumerate}

\subsection{Settings}
Continual learning has been studied within three distinct scenarios \cite{hsu2019reevaluating, vandeven2019scenarios}:

\begin{enumerate}
    \item Task-Incremental Learning: In this model, an algorithm continually acquires knowledge from distinct tasks. The algorithm is always aware of the specific task it needs to handle. Task-specific elements or even dedicated networks can be established for each task to avoid forgetting. However, efficient cross-task sharing of learned information for performance improvement and using insights accumulated from one task to boost the performance of others prove to be challenging.
    \item Domain-Incremental Learning: Under this setup, the algorithm persistently learns from an unchanging problem structure but from variable contexts or input-distributions. While the algorithm consistently masters tasks or 'domains', there's no clear demarcation of what task a sample belongs to during testing. Minimizing forgetting is particularly challenging in this context. 
    \item Class-Incremental Learning: This approach involves an algorithm gradually learning to differentiate between an increasing assortment of objects or classes. The process includes handling a range of classification tasks that require the algorithm to both detect the task to which a sample belongs and to successfully complete it. The central obstacle here is the learning to differentiate between classes that are not jointly observed, a considerable hurdle for deep neural networks, particularly when saving examples from classes seen in the past is forbidden.
\end{enumerate}

\subsection{Approaches:}

Various approaches have been investigated to address the challenges associated with continual learning. They can be categorized into the following broad categories \cite{wang2023comprehensive, Delange_2021}:

\subsubsection{Replay based approaches:}
    \begin{enumerate}
        \item Experience Replay: It stores selected previous training samples in a small memory buffer \cite{chaudhry2019tiny}. Challenges involve the careful selection and update of old training samples in the replay buffer. 
        \item Generative Replay: An additional generative model is trained to generate replay data \cite{generative1, generative2}. Various types of generative networks like Generative Adversarial Networks (GANs) and Variational Autoencoders (VAEs) have been explored. 
        \item Feature Replay: This retrieves the distribution of old features using prototypical examples.  
    \end{enumerate}
\subsubsection{Regularization based approaches}
Two primary approaches have been studied under the umbrella concept of regularization-based learning in models. Firstly, weight regularization \cite{zenke2017continual, Kirkpatrick_2017} imposes penalties on the loss function to preserve certain network parameters. Many approaches have been investigated in coming up with ways to measure parameter importance for each task.  The second set of regularization-based approaches leverages techniques like knowledge distillation \cite{Gou_2021} using older training samples to address the issue of catastrophic forgetting. 

\subsubsection{Architecture based approaches}
These approaches focus on splitting parameters into task-specific groups to avoid inter-task inference and prevent catastrophic forgetting. Various techniques like modular networks \cite{rusu2022progressive}, task specific parameter allocation and decomposing the model into shared and independent modules helps mitigate catastrophic forgetting \cite{ebrahimi2020adversarial}. However, these approaches face difficulties with scalability and sharing knowledge across tasks. 

\subsubsection{Optimization based approaches}

These approaches focus on investigating optimization techniques that align/constrain \cite{gem1, gem2} parameter updates with past data to prevent catastrophic forgetting. It has also been found that last scale pre-training can help prevent catastrophic forgetting due to more robust representations. 

\subsection{Continual learning at scale}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.5\textwidth]{intro_figs/scaling_transfer.pdf}
    \caption{The effect of scale on effect data transferred. Effective data transferred is the extra amount of data a model of the same size would need, to achieve the same performance when training from scratch, instead of fine-tuning a pretrained model. \cite{2021arXiv210201293H}}
    \label{fig:scale-transfer}
\end{figure}

Various recent studies \cite{2021arXiv210201293H, ramasesh2022effect, scialom2022fine} have investigated continual learning at scale. In \cite{2021arXiv210201293H}, the authors investigate and study the scaling laws for transfer. They study the amount of effective data transferred when fine tuning a pretrained model on a new distribution. Effective data transferred is the extra amount of data a model of the same size would need to achieve the same performance when training from scratch. As seen in Fig. \ref{fig:scale-transfer}, it was found that the effective data transferred improves as the model size increases. They also find, as shown in Fig. \ref{fig:ossification}, that small models when fine tuned on an amount of data larger than needed, they start to face the phenomenon of “ossification”, and it's better to train a model from scratch on the new dataset, i.e. pretraining can hurt performance. 

\begin{figure}[!h]
    \centering
    \includegraphics[width=0.8\textwidth]{intro_figs/ossification.pdf}
    \caption{Ossification: In the high data regime, it is observed that one can get better performance training models on larger size datasets (>1e8) from-scratch instead of fine-tuning pretrained models. \cite{2021arXiv210201293H}}
    \label{fig:ossification}
\end{figure}



In \cite{ramasesh2022effect}, it was found that pretrained foundation models face much less catastrophic forgetting compared to models trained from scratch. They find that as one scales up the model and pre-training dataset size, the degree the model faces catastrophic forgetting reduces as shown in Fig. \ref{fig:scale-forgetting}. It was found that this is due to class representations of distinct classes in pretrained models being more orthogonal and robust helping avoid interference between classes. In another study, Continual-T0 (CT0) \cite{scialom2022fine}, explores the capability of large language models to learn a myriad of tasks by fine-tuning on natural language instructions while avoiding catastrophic forgetting of previous tasks. It was found that using a very small memory buffer containing only 1\% of past data was good enough to maintain almost 100\% of the training performance on all previous tasks. CT0 is built on a T0 model, initially trained on 50 datasets. The base model is then trained on 8 new tasks while preserving past capabilities. 

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\textwidth]{intro_figs/scaling_forgetting.pdf}
    \caption{\textbf{Forgetting frontier across model scales}: Task A versus Task B performance for both pretrained vision transformers (left) and ResNets (center). Each point represents a different choice of learning rate or finetuning step for Task B. All models were pretrained on ImageNet21k for 90 epochs. (right) the best average Task A/B error improves systematically with model size \cite{ramasesh2022effect}}
    \label{fig:scale-forgetting}
\end{figure}

% \bibliographystyle{plain-fr} % style plain francais
%%\bibliographystyle{<style>} % autre
% \sectionbibliography{ref.bib} %Donner le nom du .bib
\endinput
%%
%% End of file `introduction.tex'.
